A Blockchain based and GDPR-compliant design of a system for digital education certificates

Blockchain is an incipient technology that offers many strengths compared to traditional systems, such as decentralization, transparency and traceability. However, if the technology is to be used for processing personal data, complementary mechanisms must be identified that provide support for building systems that meet security and data protection requirements. We study the integration of off-chain capabilities in blockchain-based solutions moving data or computational operations outside the core blockchain network. We develop a thorough analysis of the European data protection regulation and discuss the weaknesses and strengths, regarding the security and privacy requirements established by that regulation, of solutions built using blockchain technology. We also put forward a methodological framework that helps systems designers in combining operational off-chain constructs with traditional blockchain functionalities in order to build more secure and privacy aware solutions. We illustrate the use of that framework presenting and discussing the design of a system that provides services to handle, store and validate digital academic certificates.

==> relwork.tex <==
\section{Related work} 
\label{relwork}
There exist several proposals for off-chain solutions, the most common ones being either an external datastore, an external server or an external peer-to-peer network. In \cite{SOK} two differente off-chain models are proposed. The \textit{distributed or channels} model  consist of a group of equal nodes in a peer-to-peer network outside the blockchain, which are organized by pre-defined rules. The \textit{commit-chains or centralized}  model consists of a centralized system which receives and processes user requests and periodically responds to the chain.  The result of the procesing is transmitted to the blockchain, which in turn verifies the result before persisting it. In order to carry out that verification without disclosing confidential information the use of zero-knowledge test and verification process like zk-SNARKs~\cite{zkSNARKs} and zk-STARK~ \cite{10.1109/Cybermatics_2018.2018.00199} has been proposed.
An off-chain solution may also be conceived as a storage or external processing system or as an hybrid one~\cite{10.1145/3284764.3284766}. In \cite{10.1007/978-3-319-67262-5} different off-chain processing patterns are proposed.  In this paper we put forward a consolidated understanding of those proposals providing guidelines to select offchain models and their corresponding architectures and  technologies according to the problem to be solved 
%
Some of the challenges concerning data protection requirements the GDPR regulation poses to solutions built using blockchain technology are discussed in \cite{EPRS-art29} and \cite{EUBOF}. In those works it is analyzed the processing of pseudoanonymised and anonymized data and the potential privacy violations that might occur from the use of hash values and private/secret keys in blockchain solutions.  In \cite{DBLP:journals/corr/abs-1902-06359},  \cite{DBLP:journals/corr/abs-1904-03038} and \cite{10.1109/SC2.2018.00018}, different software architecture are proposed and discussed that have been conceived to make use of blockchain mechanisms to perform access control to data and auditing and to use off-chain solutions to safely storage and process  personal data. We propose to use additionally the blockchain as an integrity network in order to validate data stored off-chain, a link to data that is stored off-chain network is kept in the blockchain network so that it is possible to locate the data. Together with this information, it can be stored an integrity control check mechanism, for instance using a hash function.

In this paper we also put forward a methodological framework to specify the behavior and services of a system that integrates blockchain and off-chain functionalities. The two main components of the framework are a software architecture model and a use case model, which have been conceived to provide support for the construction of systems that are GDPR compliant by design. 

We illustrate the use of the proposed framework providing insights on  the implementation of a prototype of a system that provides functionalities to handle, store and validate academics digital certificates.

%Additionally, we carried out an analysis of the GDPR regulation, in order to determine the weaknesses and strengths of blockchain against personal data protection laws. In this analysis there are several subjective points, like those analyzed by \cite{EPRS-art29} and \cite{EUBOF}, related to pseudonymisation and data anonymization in the use of hash and public/private keys. From this analysis, we categorize which offchain or blockchain architecture model is recommended to select, in order to comply with GDPR.
%%
%Finally, we focus on analyzing possible architectures GDPR compliance, like ~

Based on these models we propose an architecture that incorporates some of the concepts presented, adding the integrity check functionality, even as a standalone functionality and we also propose some implementation considerations that should be taking into account, since there are requirements in GDPR that are not satisfied by design. About this architecture we propose 8 uses cases, included the verification operation that does not require access to the data itself. This operation is of special importance for the completeness of the proof of concept proposed later. In this use cases we analyze the relationship that should exist between the owner, the data controller and the data processor, according to the GDPR requirements. 

%Taking these criteria into consideration, we proposed a framework to select offchain models and architectures, as well as technology, according to the problem to be solved. 

%Additionally, we carried out an analysis of the GDPR regulation, in order to determine the weaknesses and strengths of blockchain against personal data protection laws. In this analysis there are several subjective points, like those analyzed by \cite {b10} and \cite {b11}, related to pseudonymisation and data anonymization in the use of hash and public / private keys. From this analysis, we categorize which offchain or blockchain architecture model is recommended to select, in order to comply with GDPR.

%Finally, we focus on analyzing possible architectures GDPR compliance, like ~\cite{DBLP:journals/corr/abs-1902-06359}, ~\cite{DBLP:journals/corr/abs-1904-03038} and ~\cite{10.1109/SC2.2018.00018}, that propose different architecture to use blockchain to perform certain operations related to access control and auditing and to use offchain to storage personal data or compute process related to personal data. 
%Based on these models we propose an architecture that incorporates some of the concepts presented, adding the integrity check functionality, even as a standalone functionality and we also propose some implementation considerations that should be taking into account, since there are requirements in GDPR that are not satisfied by design. About this architecture we propose 8 uses cases, included the verification operation that does not require access to the data itself. This operation is of special importance for the completeness of the proof of concept proposed later. In this use cases we analyze the relationship that should exist between the owner, the data controller and the data processor, according to the GDPR requirements. 

